IDentity with Locality: An ideal hash for gene sequence search

Gene sequence search is a fundamental operation in computational genomics. Due to the petabyte scale of genome archives, most gene search systems now use hashing-based data structures such as Bloom Filters (BF). The state-of-the-art systems such as Compact bit-slicing signature index (COBS) and Repeated And Merged Bloom filters (RAMBO) use BF with Random Hash (RH) functions for gene representation and identification. The standard recipe is to cast the gene search problem as a sequence of membership problems testing if each subsequent gene substring (called kmer) of Q is present in the set of kmers of the entire gene database D. We observe that RH functions, which are crucial to the memory and the computational advantage of BF, are also detrimental to the system performance of gene-search systems. While subsequent kmers being queried are likely very similar, RH, oblivious to any similarity, uniformly distributes the kmers to different parts of potentially large BF, thus triggering excessive cache misses and causing system slowdown. We propose a novel hash function called the Identity with Locality (IDL) hash family, which co-locates the keys close in input space without causing collisions. This approach ensures both cache locality and key preservation. IDL functions can be a drop-in replacement for RH functions and help improve the performance of information retrieval systems. We give a simple but practical construction of IDL function families and show that replacing the RH with IDL functions reduces cache misses by a factor of 5x, thus improving query and indexing times of SOTA methods such as COBS and RAMBO by factors up to 2x without compromising their quality. We also provide a theoretical analysis of the false positive rate of BF with IDL functions. Our hash function is the first study that bridges Locality Sensitive Hash (LSH) and RH to obtain cache efficiency.

==> algorithms/abf.tex <==
\begin{algorithm}
% \setstretch{1.14}
\begin{algorithmic}
\STATE {\bf INSERT: Array of \name-BF }
% $\psi: U\rightarrow m+L$: \name hash function
% $\rho :U \rightarrow [L]$ 
\STATE {\bf Input:} $\{G\}_{i =1}^{N}$: $N$ species genomes, $\{\mathbb{B}\}_{i =1}^{N}$: set of \name-BF 
\FOR{ $i \in 1..N$}
    \STATE $\mathbb{B}_i \leftarrow$ \name-BF INSERT($G_i$)\\
\ENDFOR
\STATE
\STATE {\bf QUERY: Array of \name-BF }
\STATE {\bf Input:} $Q$: query string, $\mathbb{B}_{i =1}^{N}$: Indexed set of \name-BF 
\STATE Init: Membership = $\mathbf{0}[N]$
\FOR{ $i \in 1..N$}
   \STATE Membership[$i$] = \name-BF QUERY($\mathbb{B}_i$)\\
\ENDFOR
 \end{algorithmic}
  \caption{Insert and query on Array of \name-BF}
  \label{alg:ABFInsertQuery}
\end{algorithm}

==> algorithms/overall.tex <==
\begin{algorithm}
% \setstretch{1.14}
\begin{algorithmic}
\STATE {\bf \name-BF INSERT}
% $\psi: U\rightarrow m+L$: \name hash function
% $\rho :U \rightarrow [L]$ 
\STATE {\bf Input:} $G$: genome string, $\mathcal{M}: MinHash$, $\rho \in \mathcal{R}$: random function, $k$: kmer size, $t$: sub-kmer size, $\mathbb{B}$: \name-BF of size $m$
\STATE $\{x_i\}_{i=1}^{|G|-k+1}= \mathcal{S}(G, k)$\\
\STATE Init  \name-BF : $ \mathbb{B} = \mathbf{0}[m]$\\
\FOR{ $i \in 1..|G|-k+1$}
    \FOR{ $j \in 1..\eta$}
        \STATE $loc_j \leftarrow \psi(x_i, t, L) = \mathcal{M}(x_i, t)+ \rho(x_i)$ : seed=  $j$ \\
        \STATE $\mathbb{B}[loc_j] = \mathbf{1}$\\
    \ENDFOR
\ENDFOR
\STATE
\STATE {\bf \name-BF QUERY}
\STATE {\bf Input:} $Q$: query string, $\mathcal{M}: MinHash$, $\rho \in \mathcal{R}$: random hash, $k$: kmer size, $t$: sub-kmer size, $\mathbb{B}$: Indexed \name-BF 
\STATE $\{q_i\}_{i=1}^{|Q|-k+1}= \mathcal{S}(Q, k)$\\
\FOR{ $i \in 1..|Q|-k+1$}
    \FOR{ $j \in 1..\eta$}
        \STATE Init:  $bit = 0$, Membership
        \STATE $loc_j \leftarrow \psi(q_i, t, L) = \mathcal{M}(q_i, t)+ \rho(q_i)$ : seed=$j$ \\
        \STATE $bit = bit \And \mathbb{B}[loc_j]$\\
        \IF{$bit == 0$}
            \STATE Membership = False\\
            \STATE EXIT\\
        \ENDIF
    \ENDFOR
\ENDFOR
\STATE Membership = True
 \end{algorithmic}
  \caption{Insert and query from \name-BF}
  \label{alg:IDLBFInsertQuery}
\end{algorithm}

% \STATE 
% \STATE 
% \STATE {\bf Input:} Set of kmers $x_1...x_n$ from a gene sequence $S$, 
% \STATE  \ \ \     $h_u(.)$ universal hash
% \STATE {\bf Result:} $h_f(x)$
% \FOR{term $i \in $ $1..n$}
%     \STATE $ h_m(x) = \min_{j} \left(h_u(x_{i,j})\right) , j \in \{1..k-d+1\} $
%     \STATE $h_m(x) = L*h_m(x)mod  \left \lceil{\frac{m}{L}}\right \rceil$
% \ENDFOR  
% \STATE $ h_f(x) = h_m(x) +  h_u(x) mod L$
    
%  \end{algorithmic}
%   \caption{Fuzzy LSH Algorithm}
%   \label{alg:fuzzyLSH}
% \end{algorithm}


% \begin{algorithm}
% % \setstretch{1.14}
% \begin{algorithmic}
% % \SetAlgoLined
% \STATE {\bf Input:} Gene sequence $S$, $h_f(.)$ fuzzy hash function
% \STATE {\bf Result:} CKBF (size: $m$ )
% \FOR{kmer $x \in $ $\mathcal{S}$}
%         \STATE $CKBF[h_f(x)]=1$
% \ENDFOR
% % \WHILE{Input $S_i$}
% %     \FOR{term $x \in $ $S_i$}
% %         \FOR{$d = 1, ... R$}
% %             \STATE Insert($x$, CKBF[$ \phi_d(x),d$])
% %         \ENDFOR
% %     \ENDFOR 
% % \ENDWHILE
%  \end{algorithmic}
%   \caption{CKBF Sequence Insert and Query. \todo{To finish}}
%   \label{alg:ckbf}
% \end{algorithm}

% \begin{algorithm}[]
% % \setstretch{1.14}
% \begin{algorithmic}
% % \SetAlgoLined
% \STATE {\bf Input:} Q :query or genome string, $k$: k-mer size, $t$: sub-k-mer size, $\rho \in \mathcal{R}:U \rightarrow [N]$. where U is the set of all k-mers and N is a large integer  \\

% \STATE $\{x_i\}_{i=1}^{|Q|-k+1} = \mathcal{S}(Q, k)$  \ \ \ \ \#set of kmers  \\
% \STATE $\{y_j\}_{j=1}^{k-t+1} = \mathcal{S}(x_0, t)$  \ \ \ \ \#set of sub-kmers \\
% \STATE $\mathbf{T} \leftarrow \textrm{min-heap}\left(\{\rho(y_j)\}_{j=1}^{k-t+1}\right)$\\
% \STATE $idx \leftarrow 0$\\

% \FOR{$x \in \{x_1, x_2, ... x_{|Q|-k+1}\}$ }
%     \STATE $y_{in} = \mathcal{S}(x, t)[-1]$  \ \ \ \ \#incoming sub-kmer\\
%     \STATE $y_{out} = T[idx]$  \ \ \ \ \#outgoing sub-kmer \\
%     \STATE $\textrm{update-tree}(T, y_{out}, y_{in})$
%     \STATE yield $T.top()$\\
%     \STATE $idx = (idx+1)\%(k-t+1)$\\
% \ENDFOR  
%  \end{algorithmic}
%   \caption{Rolling-min-hash over k-mers of gene string in case of full min-tree ($k{-}t{+}1$ is power of 2.)\gaurav{anyone knows how to put comments right aligned?}}
%   \label{alg:rollingmh}
% \end{algorithm}

==> figures/single_bf_and_abf_vs_fpr.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[0.48\textwidth]
  \includegraphics[scale=0.5]{imgs/single_bf_vs_fpr_new.png}
  \end{subfigure}
  
  \includegraphics[scale=0.5]{imgs/single_bf_vs_fpr_new.png}
  \caption{[Left 3: \name-BF vs BF] The impact of varying false positive rate of \name-BF vs BF on query time, indexing time, and BF size. Points towards the lower left are better. \name-BF consistently outperforms BF by achieving lower query and indexing time for the same or better FPR. [Right 3: \name-ABF vs ABF] The impact of varying false positive rate of \name-ABF vs ABF on query time, indexing time, and BF size. Points towards the lower left are better. \name-ABF reduces query time by up to $27.7\%$ and indexing time by up to $33.8\%$ while achieving the same or better FPR.}
  \label{fig:single_bf_and_abf_fpr}
\end{figure*}

==> new_sections/experiments.tex <==
In this section, we demonstrate the effectiveness of \name-BF and \name-ABF over the baselines BF and ABF respectively for gene sequence search. 
%We extend \name-BF to support multiple set membership testing by introducing Array of \name-Bloom Filters (\name-ABF).
We perform the experiments on RAM measuring index, query times and false positive rates (FPR). Additionally, we also perform experiments for inset and query on disk. 
% as all bloom filters for petabytes of genomic data cannot lie on RAM where the cache/page efficiency is even more important.

% First, we compare \name-BF with Bloom Filter when residing in RAM on the set membership testing task. Then, we compare Array of \name-BF with Array of Bloom Filters on the multiple set membership testing task. We compare them in two settings, in RAM and on disk to reflect real-world use scenarios. Finally, we demonstrate the potential gains in efficiency and reduction in false positive rate of Array of \name-BF in large-scale genome search applications by performing gene search on $1.2$TB of real-world genomic data. 


% \begin{figure}
%   \centering
%   \includegraphics[scale=0.5]{imgs/single_bf.png}
%   \caption{The impact of different sizes of \name-BF vs BF on the metrics. Query Time and indexing time grows significantly slower for \name-BF when compared with BF, with similar similar FPR. \gaurav{BF size ; mention GB/MB..}}
%   \label{fig:single_bf}
% \end{figure}

\input{figures/panel2}

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.5]{imgs/single_bf_fpr.png}
%   \caption{The impact of varying false positive rate of \name-BF vs BF on time spent per query and per item indexed. Points towards the lower left are better. \name-BF consistently outperforms BF by achieving lower query and indexing time for the same or better false positive rate.}
%   \label{fig:single_bf_fpr}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[scale=0.25]{imgs/abf_disk_vs_size_new.png}
%   \caption{The impact of different total sizes of \name-ABF vs ABF on query time and indexing time, when using disk. The growth of query time for \name-ABF is almost flat while ABF grows much faster, thanks to its cache efficient design. \name-ABF is consistently more efficient in query time than BF for the same or better FPR. \name-ABF reduces query time by up to $29.0\%$ while achieving the same or better FPR.}
%   \label{fig:abf_disk_combined}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.5]{imgs/abf_ram_vs_fpr.png}
%   \caption{The impact of varying false positive rate of Array of \name-BF vs Array of Bloom Filters on time spent per query and per item indexed, when residing on RAM. Points towards the lower left are better. For achieving the same or lower false positive rate, \name-BF reduces query time by up to $27.7\%$ and indexing time by up to $33.8\%$.}
%   \label{fig:abf_ram_vs_fpr}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.5]{imgs/abf_disk_vs_size.png}
%   \caption{The impact of different sizes of Array of \name-BF vs Array of Bloom Filters on the metrics, when residing on disk. The growth of query time for \name-BF is almost flat while BF grows much faster. Two algorithms have similar FPR across different BF sizes.\gaurav{
%   use markers in plots. triangle- BF, circle-\name-BF
%   https://matplotlib.org/stable/api/markers_api.html
%   }}
%   \label{fig:abf_disk_vs_size}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.6]{imgs/abf_disk_vs_fpr.png}
%   \caption{The impact of varying false positive rate of Array of \name-BF vs Array of Bloom Filters on time spent per query, when residing on disk. Points towards the lower left are better. \name-BF is consistently more efficient in query time than BF for the same false positive rate. For achieving the same or lower false positive rate, \name-BF reduces query time by up to $29.0\%$.}
%   \label{fig:abf_disk_vs_fpr}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[scale=0.55]{imgs/ablation.png}
%   \caption{Ablation Study.We show the impact of BF size, number of hash functions $\eta$, length of subkmer size $t$ and \name random hash range $L$ on FPR and query time. \gaurav{tip: change legend hash time per query to "Hash Time", BF False positive rate to "BF FP rate"}}
%   \label{fig:ablation}
% \end{figure}

% highlight significant boost in indexing time
% brute force match is very time-consuming, bioinformatics data volume, 

\textbf{Dataset:} We use randomly selected FASTQ\cite{FASTQ} sequence files microbial genome database
%created by Bradley et.al.
\cite{bigSI}. 
%Given the file names, the raw sequence files are
Data is downloaded using the SRAToolkit\cite{SRAToolkit} provided by NCBI. These files are all included in the European Nucleotide Archive (ENA) \cite{ENA2022}. For single set membership testing, we randomly sample a file from the database, while for MSMT, we randomly sample 10 files. The database of gene sequences does not provide a query set of sequences. Therefore, we generate the queries with 1-poisoning attack: for each sequence in a file, we randomly sample a subsequence of length greater than $32$, and poison the subsequence by changing one character at a random location. This process generates difficult queries for set membership testing since each query will maximally resemble to inserted sequences.

\textbf{Hardware and Software Implementation:}
All experiments are performed on a Ubuntu 20.04 machine equipped with 2 AMD EPYC 7742 64-core processors and 1.48TB of RAM. The code is written in C++ and compiled using the GNU Compiler.

\textbf{Baseline Methods:} 
We use Bloom filter (BF) and Array of Bloom Filters (ABF) as the baseline methods of \name-BF and \name-ABF, respectively.
%Bloom filters are widely employed as a means for approximate set membership testing, for its desirable properties of query efficiency, low false positive rate, and no false negatives. 
For BF and ABF, we use the general purpose MurmurHash\cite{murmur} as the hash function. The efficiency and hashingn quality of MurmurHash  makes it a strong baseline.

\textbf{Evaluation Metrics:} We use three evaluation metrics: \textbf{Index Time}: is the per item real-time during indexing one or multiple sequences. \textbf{Query Time:} per item real time to query from the data structure. \textbf{False positive rates(FPR):} We use FPR for MT and MSMT as defined in section \ref{subsec:genesearch}

 % Both indexing time and query time consist of two parts, hash time and bit WRITE/READ time in the Bloom filter. They are the lower the better.
 
 % Indexing time and query time measure the efficiency of the data structures for membership testing, and they are the lower the better. To keep the comparison straightforward across different data files, we report the indexing time per item and the query time per query in the experimental results.



% \subsection{Single Bloom Filter for Set Membership Testing}
\subsection{Results for \name-BF and \name-ABF}
Figure \ref{fig:single_bf_and_abf_size} and \ref{fig:all_vs_fpr} shows the experimental results of \name-BF vs BF and \name-ABF vs ABF. In figure \ref{fig:single_bf_and_abf_size}, we increase the size of BF and the total size of ABF to investigate its effects on the evaluation metrics. We make the following observations.
\begin{itemize}[leftmargin=*]
    \item \textbf{Low FPR} As the size of BF and ABF grows, the FPR are expected to decrease because distinct items are less likely to be hashed to the same location, leading to less hash collisions. We observe that the FPR's decrement is similar between \name-BF and BF, as well as between \name-ABF and ABF. This implies our proposed hash function has the desirable property of having similarly low collision rates like MurmurHash. \name-BF has a slightly higher FPR than vanilla BF and ABF, which is expected because \name preserves locality. This slightly worse FPR is compensated by the fact that \name-based BF achieves significant reductions in both query time and indexing time and hence can be run at higher values of bloom filter sizes to achieve same FPR at latency advantage (see figure \ref{fig:all_vs_fpr}). 
    \item \textbf{Significant Reductions in Query and Indexing Time} For indexing time, single \name-BF achieves up to 51.9\% reduction while \name-ABF achieves up to 28.6\% when compared to baselines. For query time, single \name-BF achieves up to 46.7\% reduction while \name-ABF achieves up to 33.1\% when compared to baselines. We note that the growth rates of query time and indexing time of \name-BF and \name-ABF are significantly slower than BF and ABF, respectively. This is due to the fact that larger ranges of BF and ABF result in a higher number of cache misses and page faults during indexing and querying. The efficiency advantage is more clear in the larger sizes of BF and ABF, meaning \name-BF and \name-ABF are particularly suited for large-scale set and multi-set membership testing.
\end{itemize}
The gains of \name-BF and \name-ABF in the evaluation metrics are clear with varying BF size. But what are the absolute gains in query and indexing efficiency of \name-BF and \name-ABF while achieving the same or better search quality as baselines? The results are shown in figure \ref{fig:all_vs_fpr}, which shows the querying and indexing time reductions of \name-BF and \name-ABF over baselines while achieving the same or better FPR. For almost all FPR, \name-BF and \name-ABF are able to achieve lower querying and indexing time over baselines. We highlight that \name-ABF achieves up to $27.7\%$ reduction in query time and up to $33.8\%$ reduction in indexing time over baselines while achieving better FPR. With the low FPR and significant reductions in query and indexing time combined, our proposed algorithms translate to significant efficiency gains in real retrieval applications while maintaining search quality. In applications such as gene search, terabytes of data need to be indexed and queried efficiently, \name-based BF will have a tremendous impact on the efficiency of gene search.

\subsection{Results for \name-ABF on Disk}
The rightmost plot of figure \ref{fig:abf_disk_combined} shows the experimental results of \name-ABF vs ABF, when residing on disk. Indexing time are omitted from these plots since indexing is only done on RAM in real use cases. When using the initial smaller sizes of \name-ABF and ABF, they have similar query time. However, as the total size grows, the query time of ABF quickly outgrows \name-ABF since the query time of \name-ABF remains relatively flat. At the largest size, \name-ABF on disk achieves $43.9\%$ reduction in query time than the baseline. The FPR of \name-ABF is similar or slightly higher when compared to ABF, and the significant advantage in the query time offsets the minor difference and achieves a net efficiency gain. This efficiency gain is visualized in the rightmost plot of figure \ref{fig:all_vs_fpr}, \name-ABF is always able to achieve lower query time while maintaining the same or better FPR as the baseline. \name-ABF achieves up to $29.0\%$ reduction in query time while achieving better FPR than the baseline.


%Set membership testing refers to the problem of determining if an item belongs to a set of items.  In the application of gene search, a sequence is considered to belong to a set of sequences if that sequence is a subsequence of any sequence in the set.

%We evaluate \name-Bf and Bloom filter on gene sequence search with a randomly sampled FASTQ file from the microbial genome files. We generate the query sequences with 1-poisoning attack: for each sequence in the file, we randomly sample a subsequence of length greater than $32$, and poison the subsequence by changing one character at a random location. This process generates difficult queries for membership testing, since each query will maximally resemble sequences from the original set.

% We evaluate the set membership testing performance of CKBF on the 100 FASTQ files. The CKBF and Bloom filter are compared on performance metrics: kmer query time \ref{}, kmer false positive rate \ref{}, and indexing time, while keeping the same parameters $N$ and $K$. 

% The indexing time consists of two parts hash-time (time taken for computing hash code) and write-time (on RAM/disk). Similarly, the query time involves hash-time and read-time. 

% The performance metrics

\subsection{Ablation Study}
\input{figures/panel3}
In this ablation study, we perform experiments to study the effects of all the free parameters of \name on FPR and query time of \name-BF. We list the tunable parameters of \name-BF as follows:

\begin{itemize}[nosep, leftmargin=*]
    \item the number of bits $m$ in the array underlying the Bloom filter,
    \item the number of \name hash functions $\eta$ used for the Bloom filter,
    \item the length of sub-kmers $t$,
    \item and the range $L$ of random hash in \name.
\end{itemize}

We choose a set of parameters for \name-BF that achieves less than $10^{-3}$ FPR while achieving good efficiency as the base parameters, and vary the free parameters to study the effects they have on FPR and query time. The results are shown in figure \ref{fig:abf_disk_combined}. We make the following observations.

\begin{itemize}[leftmargin=*]
    \item \textbf{The Trend of FPR} The FPR is expected to decrease with increasing $m, t$ or $L$, while FPR initially decreases then increases as $\eta$ increases. With increasing BF size $m$ or \name random hash range $L$, the hash collision rate decreases hence reducing the FPR. With increasing sub-kmer length $t$, two random kmers are less likely to share common sub-kmers, effectively decreasing the locality property of \name. On the hand, increasing $\eta$ decreases the probability of two items sharing the same hash codes, but increases the amount of bits set to $1$ in the BF.
    \item \textbf{The Trend of Query Time with $m$ and $\eta$} The query time is expected to increase monotonically with $m$ and $\eta$. Increasing the BF size $m$ increases the amount of cache misses and page faults, leading to higher query time. Increasing the number of hash functions $\eta$ increases amount of hash calls and check operations, hence increasing the query time.
    \item \textbf{High Value of $L$ Leads to Page Faults} By using values of $L$ less than $16$, \name-BF achieves similar query time, but there is a significant increase in query time when going from $L=15$ to $L=16$. This can be interpreted as more page faults during querying. Since the page size in our system is $2^{15}$ bits, increasing $L$ beyond that will result in significantly more page faults, leading to much higher query time. Therefore, we recommend using values of $L$ at or slightly below the page size to achieve the best search quality and efficiency.
    \item \textbf{The Trend of Hash Time with $t$} The length of sub-kmers $t$ heavily affects the hash time of \name. Going from $t=12$ to $t=16$ leads to a significant drop in hash time, which in turn decreases query time. This is due to the use of segment tree in our implementation for efficient computation of the minimum operation (see Algorithm \ref{alg:rollingmh}). Increasing $t$ from $12$ to $16$ reduces the size of the segment tree by more than half, thus reducing the amount of computation during hash operations. Therefore, we recommend using $t=16$ for kmer size of $31$ for striking a balance between cache efficiency and low computational overhead.
    \item \textbf{Choice of $\eta$} We compare the FPR of \name-BF with BF with increasing number of hash functions $\eta$ increases in the top right plot of figure \ref{fig:abf_disk_combined}. The two curves are closely aligned, implying \name-BF and BF behaves similarly with the same choice of $\eta$. Therefore, we recommend setting $\eta$ of \name-BF to the optimal value of $\eta$ in the BF using a random hash function, and try adjacent values of $\eta$ for parameter tuning.
\end{itemize}

% We perform membership testing with two sets of gene sequences sampled from the Whole Genome Sequencing data corpus. We set the initial parameters $m, \eta$ of \name-BF to be the optimal values used for vanilla Bloom filter, then we vary the parameters around the optimal ones and observe the effects of the changes. For the locality parameter $L$, we initially set it to be the size of the cache line, then we half or double the value of $L$ multiple times. For the length of sub-kmers $t$, we are testing all the values between $4$ and $28$ in intervals of $4$s.

==> new_sections/genesearch.tex <==
\subsection{Gene search with Bloom Filter}
Given a DNA string for query, $Q$, the task is to determine if the query $Q$ belongs to given species represented by its full-length genome $G$. The gene string of the full-length genome $G$ is usually very large, with an average length of $100$ Million \cite{gupta2021fast}. Given this large genome length, it is practically infeasible to precisely match the string. Additionally, it is useful to understand how much of the given query gene string $Q$, if not all, matches with a given Genome $G$. The standard practice to address this is to represent the genome $G$ as a set of $k$ length k-mers \cite{kmerSelection}

Given a gene string, say $G$ ( and $Q$), we divide this string into a sequence of substrings of $k$ base pairs called k-mers using a moving window. This is illustrated in figure \ref{fig:ckbf}. Let this sequence be generated by function $\mathcal{S}(.)$, 
\begin{equation}
    \mathcal{S}(G, k) = \{G[i:i+k]\}_{i=1}^{(|G| - k)}
\end{equation}

\begin{equation}
    \mathcal{S}(Q, k) = \{Q[i:i+k]\}_{i=1}^{(|Q| - k)}
\end{equation}

The Membership Testing and Multiple Set Membership Testing (MSMT) of a gene string query $Q$, is defined as follows,
\begin{definition} (Membership Testing of $Q$ in $G$)
A gene string $Q$ is said to be present in a genome of a species $G$ if the following holds,
\begin{equation}
    \mathcal{S}(Q, k) \subseteq \mathcal{S}(G, k)
\end{equation}
\end{definition}

\begin{definition} (MSMT of $Q$ in $\{G_i\}_{i=1}^N$ )
A gene string query $Q$ is said to be present in the genome of a set of species $\{G_j\}$, 
\begin{equation}
    \forall jj \in [N],  \mathcal{S}(Q, k) \subseteq \mathcal{S}(G_j, k)
\end{equation}
\end{definition}
Each of this membership-testing problem can be approximately solved using BF. In fact, BF and its variants are the state-of-the art solutions to membership testing problem in gene search. In this paper we improve the efficiency of BF based solutions for gene search by introducing new class of hash functions - \name.


==> new_sections/subsectionFig.tex <==
\begin{figure*}[h]
\centering
% \begin{minipage}{0.33\textwidth}
\subfigure[Recall10@10 vs Query Time]{
 \includegraphics[width=0.32\linewidth]{plots/sift-p50_RecallVark10@10.png}
 
 \label{fig:recall-vs-query-time}
 }
% \end{minipage}
% \hfill
% \begin{minipage}{0.33\textwidth}
\subfigure[Recall10@10 vs. NNZ(k)]{
\includegraphics[width=0.32\linewidth]{plots/sift-p50_Recall_k.png}
\label{fig:recall-vs-nnz-k}
}
% \end{minipage}
% \hfill
% \begin{minipage}{0.33\textwidth}
\subfigure[Query Time vs. NNZ(k)]{
\includegraphics[width=0.32\linewidth]{plots/sift-p50_QT_k.png}
\label{fig:query-time-vs-nnz-k}
}
% \end{minipage}
\caption{%
Recall10@10 and Query time (ms) vs the NNZ (number of non zero entries)- $k$, keeping the same hash code size ($M$). We see that increasing $k$ increases the Recall rate with marginal gains, however the query time increases as $O(k^2)$.
}%
  \label{fig:Recall_vark}
\end{figure*}

==> sections/Theoem1Proof.tex <==

\section{Proof of Theorem 1}
\begin{proof}
% To prove:\\
% Let $\phi$ be drawn from a $(r_1, r_2, p_1, p_2)$ sensitive LSH family say $\mathcal{L}$ and $\rho_1, \rho_2$ be drawn from a random hash family, say $\mathcal{R}_1 : V \rightarrow [m], \mathcal{R}_2: U \rightarrow [L]$ respectively. Then the family of hash functions defined by 
% \begin{align*}
%     \mathcal{I} : \{\psi(x) = \rho_1(\phi(x)) + \rho_2(x)) \}
% \end{align*}
% is a $(r_1, r_2, \frac{L-1}{L}p_1, \frac{L}{m} p_2)$ sensitive and $L$ preserving {\longname } (\name) family.

For a \name hash ${\psi \leftarrow \mathcal{I}}$ and LSH ${\phi \leftarrow \mathcal{L}}$,  the probability of not colliding but co-locating is represented as 
$$\mathbf{Pr} ((\psi(x) \neq \psi(y)) \textrm{ and } d_V(x, y) < L)$$ 
With LSH and RH, \name is given by $\psi(x) = \rho_1(\phi(x)) + \rho_2(x)$ 

\begin{align*}
   \mathbf{Pr} ((\psi(x) \neq \psi(y)) \textrm{ and } d_V(x, y) < L)
\end{align*}

\begin{align*}
    = (\mathbf{Pr}((\phi(x) = \phi(y)))+ L/m\mathbf{Pr}((\phi(x) \neq \phi(y))))* (1-\mathbf{Pr} (\rho(x) \neq \rho(y))) 
\end{align*}
For similar keys $d_U(x, y) < r_1$ then  $\mathbf{Pr}((\phi(x) = \phi(y))  \geq p_a = p_1 + (1-p_1)/m$, hence
\begin{align*}
    \geq (p_a + (1-p_a)L/m)* (1-1/L)
\end{align*}
\begin{align*}
    = (p_1 +(1-p_1)/m + (1-p_1 +(1-p_1)/m)L/m)* (1-1/L) \geq p_1(1-1/L)
\end{align*}
We prove that, $\mathbf{Pr} ((\psi(x) \neq \psi(y)) \textrm{ and } d_V(x, y) < L)
\geq p_1(1-1/L)$\\

Additionally, for dissimilar keys,
\begin{align*}d_U(x, y) > r_2, \textrm{then}  \mathbf{Pr}((\phi(x) = \phi(y))  \leq p_b \end{align*}

% \begin{align*}d_U(x, y) > r_2, \textrm{then}   \mathbf{Pr}(\|(\phi(x) - \phi(y)\| =0) \textrm{ and }  \mathbf{Pr}((\rho(x) = \rho(y))  \leq p_b/m\end{align*}
% For the $\|(\psi(x) - \psi(y)\|$ to be less than $L$

% \begin{align*}d_U(x, y) > r_2, \textrm{then}   \mathbf{Pr} \mathbf{Pr}(\|(\psi(x) - \psi(y)\| <L) \textrm{ and }  \mathbf{Pr}((\rho(x) = \rho(y))  \leq \frac{L}{m}p_b\end{align*}

\begin{align*}d_U(x, y) > r_2, \textrm{then}   \mathbf{Pr}_{\psi \leftarrow \mathcal{I}} (d_V(x, y) < L) = (\mathbf{Pr}((\phi(x) = \phi(y)) + (1-\mathbf{Pr}((\phi(x) \neq \phi(y))))*L/m 
\end{align*}

\begin{align*}
 \leq p_b + (1-p_b)*L/m 
\end{align*}
This proves that the \name-hash is $(r_1, r_2, \frac{L-1}{L}p_a, \frac{L}{m} p_b)$ sensitive and $L$ preserving for  with $pa>p_b$\\
\end{proof}



==> sections/abstract.tex <==
Bloom filter is a space-efficient probabilistic data structure used extensively in networking, distributed databases, and genomic search. In particular, they have succeeded by efficient indexing and searching through hundreds of terabytes of genomic data. 
Bloom filter uses a universal hash function to store a set elements' bit signatures. The universal hash, being fundamental, is also a default function for a dictionary/hash-lookup. It  has a uniform collision probability of two different keys. A Bloom filter with a universal hash is efficient but faces a high number of cache misses on querying and inserting multiple keys. In genomic search, the similarity of the neighboring gene string keys provides scope for increasing cache hits. With this motivation, we propose a novel hash function- Fuzzy Locality sensitive hash (Fuzzy-LSH), that translates the locality of the keys to the locality of the hash signatures. In essence, if two keys are similar, their hash codes are adjacent in memory. Additionally, a new type of Bloom filter called Cache Efficient kmer Bloom (CKBF) has been proposed that uses Fuzzy-LSH instead of the universal hash.
% we also propose a Cache efficient kmer Bloom (CKBF) for gene sequence membership testing. CKBF utilizes Fuzzy-LSH instead of a universal hash. 
With this CKBF provides a higher cache hits rate (\todo{x\%}) and \todo{x times} faster query time on gene sequences. When used in genomic search indices, CKBF also leads to a \todo{x times} speedup in query and index times.


% in many 
% -Bloom filter-based indices have shown promises in gene Sequence Search. \\
% -A sequence query utilizes a sliding window approach for getting kmer containment in the sequence file\\
% -universal hash leads to many cache misses\\
% -We have a cache-efficient hash function to utilize the spacial neighborhood of the kmers\\
% -Our work provides a genomic Bloom filter with a faster sequence query. We also show that the effect magnifies on Multiple Set Membership Testing based BF based indices.


==> sections/abstract_1.tex <==
Random hash (RH) and Locality sensitive hash (LSH) functions are two fundamental hash functions widely used in different indexing applications. While RH disregards similarities between tokens and distributes them independently, LSH overemphasizes similarity and encourages similar tokens to collide. However, in some applications, we want the hash function to co-locate similar tokens without causing them to collide. We describe a novel family called the \longname(\namens) family. \name functions promote similar tokens to lie close to each other (like LSH). However, it avoids collision among these (and other) tokens (like RH). We show a concrete application in genomic search, which benefits tremendously from this new class of hash functions. In gene sequence search, we check the membership of each k-mer (a tokenized gene substring) in the database using Bloom filters (BF). However, every subsequent k-mer is distributed randomly in traditional BF; thus, to access the bit for each k-mer, we have to fetch different pages/cache lines. Ideally, it would be efficient if bits corresponding to subsequent k-mers were stored `near' the bit for the current k-mer, and this would be an effective use of memory hierarchy. In this paper, we give a general formulation of \name family. We propose a \name family for gene search and show that it slashes our index time and query times by over 30\% while maintaining the false positive rate. We also provide a theoretical analysis of FPR of \name-BF.


==> sections/abstract_2.tex <==
Hashing is a core technique in many data mining systems, including search, retrieval, and recommendation. Random hash (RH) functions are crucial to designing memory and computation-efficient systems. However, the property of RH hash functions, critical to gaining resource advantage, is in direct conflict with general notions of ``locality" in memory access. This paper highlights this issue in gene sequence search. In gene sequence search, a popular subroutine is to check the membership of each k-mer (a tokenized gene substring) in the database using Bloom filters (BF). However, every subsequent k-mer, even though are likely very similar,  maps randomly in the memory location due to the uniformity of hash functions. As a result, the access pattern for successive k-mers requires accesing different pages/cache lines. Ideally, it would be efficient if memory access pattern corresponding to subsequent k-mers were co-located in memory in the same cache line. Processing a batch of queries with random memory access resulting in significantly higher memory latency and system slowdown. The hash function in bloom filters are oblivious to the intrinsic local similarity in gene sequence search. They are designed to distribute different input keys uniformly to different places. It is clear, that in the setting of gene sequence search, we are performing multiple queries with bloom filters where the query keys are almost similar but not exactly same. This paper describe a novel hash function called the \longname(\namens) family. \name functions are designed to place similar tokens to be mapped to close memory locations like LSH providing cache-efficiency. However, at the same time it avoids collision among tokens that are not exactly the same like RH. In this paper, we give a general formulation of \name family. We propose a \name family for gene search and show that it slashes our index time and query times by over 30\% while maintaining the false positive rate. We also provide a theoretical analysis of FPR of \name-BF.  Our hash function is the first study that bridges LSH and RH to obtain cache efficiency, our design and analysis could be of independent theoritical interest in itself. 


==> sections/abstract_3.tex <==
Hashing is a core technique in many data mining systems, including search, retrieval, and recommendation. Specifically, Random hash (RH) functions are crucial to designing memory and computation-efficient systems. However, the property of RH hash functions, critical to gaining resource advantage, is in direct conflict with general notions of "locality" in memory access. This paper highlights this issue in gene sequence search. Gene sequence search for a query sequence Q from a DNA database processed into a Bloom filter(BF) fires a sequence of BF membership testing queries on each k-mer of Q. While subsequent k-mers are likely very similar, RH being oblivious to any similarity, uniformly distributes the k-mers to different parts of potentially large BF, thus triggering excessive cache-misses and page-table accesses and causing system slowdown. This paper describes a novel hash function called the Identity w. Locality hash family, which can resolve the cache-inefficiency of processing a batch of queries with random memory access. IDL functions are designed to recognize and place similar tokens in close memory locations like LSH, providing cache efficiency. However, at the same time, it will avoid collision among tokens that are not exactly the same as RH. In this paper, we give a general formulation of IDL family. We propose a IDL family for gene search and obtain tremendous improvements in system performance. At the same BF sizes, IDL performs indexing and query operations at $\sim2\times$ speed for BF while maintaining the same false positive rates. We also provide a theoretical analysis of FPR of IDL-BF. Our hash function is the first study that bridges LSH and RH to obtain cache efficiency. Our design and analysis could be of independent theoretical interest.


==> sections/abstract_4.tex <==
{\color{blue}
DNA sequencing has wide applications in medicine, evolutionary biology, metagenomics, and more. Gene sequence search, i.e., searching for a given DNA sequence, say $Q$, in a genome database, say $D$, is a fundamental operation in computational genomics. Given the petabyte scale of genomes, it is not surprising that most gene search systems are based on hashing-based solutions developed for databases. Specifically, the state-of-the-art gene search systems such as COBS (Compact bit-slicing signature index) \cite{bigSI} and RAMBO (Random and Merged Bloom Filter) \cite{gupta2021fast} use probabilistic data structure: Bloom Filters (BF). The standard recipe is to cast the gene search problem as a sequence of membership testing for subsequent k-mers of Q in the set of k-mers of D.  We observe that usage of Random hash (RH) functions, which are crucial to exponential memory and the computational advantage of BF are also detrimental to the system performance of gene-search systems. While subsequent k-mers being queried are likely very similar, RH, oblivious to any similarity, uniformly distributes the k-mers to different parts of potentially large BF, thus triggering excessive cache misses and causing system slowdown. 


This paper describes a novel hash function called the Identity with Locality (IDL) hash family, which combines the benefits of LSH and RH functions. With high probability, the IDL function co-locates the tokens close in input space without causing them to collide. We give a simple but practical construction of IDL function families. IDL functions can be a drop-in replacement for RH functions and can help improve system performance of information retrieval systems. This paper provides an IDL function for gene sequence search, which captures the similarity between subsequent queries. We show that replacing the RH function with IDL functions reduces the cache-misses by a factor of $5\times$, thus improving query and indexing times of SOTA methods such as COBS and RAMBO by factors up to $2\times$ without compromising their quality. We also provide a theoretical analysis of the FPR of Bloom filters with IDL functions. Our hash function is the first study that bridges LSH and RH to obtain cache efficiency. Our design and analysis could be of independent theoretical interest.

==> sections/background.tex <==
\subsection{Bloom Filter}
Bloom Filter \cite{} is a data structure that represents a set $\mathcal{S}$ of $n$ items with a one-dimensional bit-array of approximately $O(n)$ size. An item can be queried from the Bloom filter to check its presence in the set $\mathcal{S}$. To represent the set of items, an array $\mathbb{B}$ of size $m$ is initialized with all bits 0. All the items  $x \in \mathcal{S}$ of the set are hashed with $\eta$ universal hash \cite{} functions $h_1(x), h_2(x),.. h_{\eta}(x)$, to get $\eta$ locations of bits to set 1. Upon query, the same hash functions $h_1(q), h_2(q),.. h_{\eta}(q)$ are used to get bit locations for the item $q$. If all the bits are 1 at these hash locations, the query $q$ is inferred as part of the set $\mathcal{S}$.

The Universal hash function used in the Bloom filter has the collision probability ($P(h(x) = h(y)), x\nq y$) upper bounded by $1/m$. The $\eta$ bits at the hash location $h_1(q), h_2(q),.. h_{\eta}(q)$ can be all be 1 even if $q \notin  \mathcal{S}$. It happens with a very small probability 
$p = \left(1-\left[1-{\frac {1}{m}}\right]^{\eta n}\right)^{\eta} \approx \left(1-e^{-\eta n/m}\right)^{\eta} $, called false positive rate. 
To minimize the false-positive rate, we use $\eta = -\frac{\log p}{\log 2}$ and $m = -n \frac{\log p}{\log 2}$.

\subsection{Universal hash property}
A set (family) of hash function $H$ is universal if by randomly choosing a hash function $h\in H$, $h: U \rightarrow {1....m}$ and for all $x\neq y \in U$
$$Pr_{h\leftarrow H}(h(x)= h(y))\leq 1/m$$

Here $m$ is the maximum value of the hash function.

\subsection{Locality Sensitive Hash}

Locality Sensitive Hashing (LSH)~\cite{Indyk1998ApproximateNN, charikar2002similarity} is a technique from computational geometry that was introduced for approximate nearest neighbor search. An LSH family $\mathcal{H}$ is a family of functions $h(\mathbf{x}): \mathcal{U}\to \mathbb{Z}$ with the following property: Under $h(\mathbf{x})$, similar points have a higher probability of \textit{colliding} (i.e. $h(\mathbf{x}_1) = h(\mathbf{x}_2)$) than dissimilar points having the same hash value.  

This implies that if the given two points $x$ and $y$ are similar, then the corresponding hash values $h(x)$ and $h(y)$ are same with high probability.
The notion of similarity is usually based on the distance measure in the metric space $\mathcal{X}$. For instance, there are LSH families for the Jaccard~\cite{broder1997resemblance}, Euclidean~\cite{datar2004locality,andoni2006near} and angular distances~\cite{charikar2002similarity}.
\begin{definition} [\bf LSH Family]\ A family  $\mathcal{H}$ is called
                $(r,cr,p_1,p_2)$-sensitive if for any two points $x,y \in \mathcal{U}$ and $h$ chosen uniformly from $\mathcal{H}$ satisfies the following:
               
                \begin{itemize}
                                \item if $Dist(x,y)\le r$ then ${Pr}(h(x) = h(y)) \ge p_1$
                                \item if $ Dist(x,y)\ge cr$ then ${Pr}(h(x) = h(y)) \le p_2$
                \end{itemize}
                \label{def:lsh}
\end{definition}
\subsubsection{\textbf{Minhash}}
MinHash is LSH function defined over a set if items. The similarity function it uses it Jaccard, which is defined as the size of the intersection of two sets say $\mathcal{S}_1$ and $\mathcal{S}_@$ divided by the size of the union of $\mathcal{S}_1$ and $\mathcal{S}_2$.
$$MinHash(\mathcal{S}) = \min{h(x) | x \in \mathcal{S}}$$
The minhash value is calculated by taking the minimum universal hash value of all the elements in the given set.



==> sections/experiments.tex <==
\subsection{Dataset}
We make use of randomly selected 100 gene sequence files that were downloaded from the \cite{} 170TB Whole Genome Sequencing data corpus. These files are all included in the European Nucleotide Archive (ENA) \cite{ENA2022}. For information on the data statistics, see Figure \ref{}. The files are available in FASTQ format. (\todo{More about FASTQ}). Addtionally, we use 4000 FASTQ files randomly selected from the same data corpus for the genomic search index. 

\subsection{Hardware}

\subsection{Evaluation Metrics}

\subsection{Baseline Methods}


\subsection{Single Bloom Filter for Set Membership Testing}

We evaluate the set membership testing performance of CKBF on the 100 FASTQ files. The CKBF and Bloom filter are compared on performance metrics: kmer query time \ref{}, kmer false positive rate \ref{}, and indexing time, while keeping the same parameters $N$ and $K$. 

The indexing time consists of two parts hash-time (time taken for computing hash code) and write-time (on RAM/disk). Similarly, the query time involves hash-time and read-time. 

The performance metrics

\subsection{Array of Bloom Filters for Multiple Set Membership Testing}
The improved query time of CKBF also impacts a multiple-set membership testing-based genomic search engine. We do a case study on Array of Bloom filters (\ref{}\todo{bigsi and cobs}) and analyze the index on the number of files varying from 100 to 4000.


\subsection{Ablation Study}

In this ablation study, we will study the effects of all the parameters of \name on the false positive rate, indexing time, and query time of bloom filters. We list the tunable parameters of \name-BF as follows:

\begin{itemize}
    \item the number of bits $m$ in the array underlying the Bloom filter,
    \item the number of \name hash functions $\eta$ used for the Bloom filter,
    \item the locality parameter $L$,
    \item and the length of sub-kmers $t$.
\end{itemize}

We perform membership testing with two sets of gene sequences sampled from the Whole Genome Sequencing data corpus. We set the initial parameters $m, \eta$ of \name-BF to be the optimal values used for vanilla Bloom filter, then we vary the parameters around the optimal ones and observe the effects of the changes. For the locality parameter $L$, we initially set it to be the size of the cache line, then we half or double the value of $L$ multiple times. For the length of sub-kmers $t$, we are testing all the values between $4$ and $28$ in intervals of $4$s.


\newpage


Math Equations

\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}


==> sections/introduction.tex <==
A Gene sequence or DNA is a long strand of four chemical bases: adenine (A), guanine (G), cytosine (C), and thymine (T), found in living cells and viruses. The arrangement of A,T,C and G in the DNA uniquely encodes a species' specific build-up, biological properties, and function. These gene sequences of the known species are read and stored for biological research and analyses via sequencing machines. The European Nucleotide Archive (ENA) \cite{ENA2022}, and NCBI have documented a total of ---Petabytes of DNA sequences. 
The sheer scale has geared up innovation for efficient sequence databases and search algorithms. Many existing algorithms use a kmer-based gene representation. Like an n-gram token for a text, kmer is usually a $k$ length token generated using a sliding window of stride one on the sequence \ref{fig-kmer}. This bag of kmer representation of a sequence is used ubiquitously \cite{}. With this, the gene sequence is encoded in a Bloom Filter \cite{} \ref{section-BF} in many state-of-the-art search engines \cite{}. A single gene sequence can be as large as X billion for -- and usually 50-200M in length in a single parasite and bacteria. Having millions of species in archives, a Bloom filter serves as a cheaper and fast to query data structure for membership testing. 

\todo{to make: 1) sequence to kmer and query processing figure, 2) Bloom filter index structures}

The existing state of art indices \cite{bigsi} \cite{cobs} \cite{ssbt} \cite{RAMO} uses Bloom filter as a building block membership tester to provide quick search results in cheap memory \ref{fig:BFdataStr}. 

We focused on improving the Bloom filter query time for a gene sequence. Given a Bloom filter representation of a gene sequence, any query of a given length ($>k$), is tested for presence by querying all constituent kmers of the query. This is shown in Figure \ref{cacheMotivation}. It is standard practice to break the query by sliding windows of length $k$ and get each kmer's membership result. The AND operation among outputs provides a full query membership test. Additionally, other metrics/cues like \todo{---define} are derived from the set of outputs. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{imgs/fuzzylsh.png}
  \caption{ }
  \label{fuzzyHashGeneric}
\end{figure}

The existing Bloom filter implementations use a universal hash function \cite{} \ref{} to represent a kmer's bit signature on the Bloom filter. This provides standard Bloom filter guarantees and performs independent Write/Read for each kmer. The biggest caveat in this setup is a high cache miss rate (figure \ref{cacheMotivation}). It is important to note that any adjacent kmers in a gene sequence differs from its neighbors by two base-pairs. We can significantly improve the cache hits if we can force a locality in hash codes for the adjacent kmers. For example, for a gene string ACCGTAG and its kmers ACCG, CCGT, CGTA, GTAG; an adjacent pair ACCG, CCGT hash codes are independent to each other and will lead to the fetch of different cache lines with high probability (--). However, forcing these hash values to fall in the same cache line will significantly reduce the WRITE/READ latency. 

\paragraph{\textbf{Why we need a Fuzzy locality sensitive hash \gaurav{or "Locality Maintaining Hash"??}} }
The universal hash provides unique separability among the keys by having a low collision probability rate for every key independently. Using this hash function, the value against the key is shared minimally against any other key.
With it, the membership test is provided distinctively for a key on a Bloom filter.
% a Bloom filter and a hash table provide signature and values, respectively, only if the exact key is queried. 

The locality-sensitive hash, on the other hand, provides separability among the dissimilar keys and, a high collision rate for keys similar to each other. This is great for applications like Near neighbor search, selective sampling, or Distance Sensitive Bloom filter \cite{}. However, LSH  dissolves/combine the values of similar keys, as they have no separability. Hence, the membership test on a Bloom filter is not distinct for similar keys.

The Fuzzy LSH maintains locality with separability! It gets the hash value of similar keys near each other but not the same with a high probability. This enjoys the best of both worlds. In sequence indexing, the  Fuzzy LSH preserves the locality of similar keys by putting them adjacent, and it preserves distinctness by keeping a different hash location for each key with high probability. 

\paragraph{\textbf{Contributions:}}
In this work, we provide a cache-efficient Bloom filter for gene string by making the following contributions- 

\begin{itemize}
    \item We provide a novel hash function - Fuzzy Locality Sensitive hash (Fuzzy-LSH), to maintain the cache line locality with intra-cache bit separability among the adjacent kmers signatures.
    \item We propose a cache efficient Kmer Bloom filter (CKBF) that utilizes Fuzzy-LSH, to improve the Insert and query time by a factor of --- on RAM and --- on disk.
    \item We analyse gene search index improvements with CKBF.
    \item We provide theoretical analysis of Fuzzy-LSH properties; CKBF's false positive and query time; and the genomicsearch index error rates.
    
\end{itemize}



==> sections/introduction_1.tex <==
% RH and LSH are super useful.  

Hash functions that map arbitrary size values to a fixed range $[m]=\{0,...m-1\}$, have been a long-researched topic and have been widely used in big data systems\cite{practicalML,b3}, network and security\cite{BFsurvey}, and AI\cite{MACH}. Specifically, Random hash (RH) and its proxies \cite{universalHashcarter1979, murmur, xxHash}, and Locality sensitive hash functions (LSH) \cite{IndykAndMotwani} have created a wave of improved probabilistic data structures which have provided exponential improvements in memory and speed with an insignificant cost of uncertainty\cite{NIPS2011_anshu}. Thus, it comes as no surprise that LSH and RH have helped to achieve performant algorithms in multiple domains, including but not limited to sampling \cite{ioffe2010improved}, retrieval \cite{IndykAndMotwani, wang2017flash, gupta2022bliss, baeza1999modern}, machine learning \cite{ryanDeepLeanring, chen2020slide}, genomic search \cite{bigSI, elworth2020petabytes}, and data analysis \cite{practicalML}.


% Missing link pros and cons midway ? spectrum.
% limitations of RH, LSH
Random Hash (RH) functions are good at maintaining the identity of the input. If two input keys are distinct, with high probability, the RH function will map it to two separate keys. While RH maintains input's identity, it is not robust to small perturbations in the input. Specifically, it does not incorporate the similarity between tokens. For example, if a user mistypes a word,  RH views it as an entirely different token. Furthermore, there are times when we want to colocate similar tokens. In such cases, locality-sensitive hash (LSH) functions are beneficial. The LSH functions map similar tokens to the same value with high probability and avoid assigning the same value for different tokens. LSH has proven very efficient for near neighbor search \cite{IndykAndMotwani} \cite{shrivastava2014asymmetric} and deep learning \cite{chen2020slide}. Nevertheless, its biggest strength is also a weakness in some applications. As LSH maps similar keys to a single value, it does not preserve the identity of these keys. In some sense, RH and LSH lie at two ends of a spectrum. LSH combines similar elements, causes them to have identical values, and induces a lapse of identity; RH preserves identity but at the cost of being agnostic to any similarity. In this paper, we provide a new hash family \longname(\name hash) that offers a way to achieve the complete spectrum between LSH and RH. We show a concrete application of \name functions in efficient search in genomic data.

%\apd{the paragraph is wordy . i am making it compact.}
% A class of hash functions- Universal hash (UH) generates a value against a key and  represents it uniquely. In essence, if any two keys are different, their corresponding hash values are different, almost certainly. This also means that the universal hash preserves the key's identity with a high probability. Assume a case of malware detection where UH provides a fast and certain solution by keeping unique hash values of a set of malwares.
% However, UH is fully agnostic to any relationship between and among keys. For example- any two strings with even a character difference will have very different hash values. This makes it less effective for detecting any unseen but lookalike malware. 
% The locality-sensitive hash (LSH) , on the other hand, provides a value shared among similar keys. In other words, the hash function has a high collision rate for keys similar to each other and a low if they are not. LSH has proven very efficient for near neighbor search \cite{IndykAndMotwani} \cite{shrivastava2014asymmetric} and deep learning \cite{chen2020slide}. Although its biggest strength is also a weakness, as it dissolves/combines the values of similar keys, they have no identity preserved. For example, detecting a cancer gene marker from a gene pool needs a highly sensitive algorithm. LSH is ineffective, but UH can gracefully address this. 

\input{figures/kmerinsert}
% paragraph on gene sequence search and that is solved using bloom filters which use LH.

The genome of an organism is the complete set of DNA for that organism. The DNA sequence readers \cite{goodwin2016coming} aim to determine the nucleic acid sequence (A, C, T, and G) of a gene. The genome archives recording such sequences for multiple species are typically very large. For instance, the European Bioinformatics Institute (EBI) has reportedly stored around 160 Petabytes of raw DNA sequences as of 2018 \cite{EBI2019}. Additionally, the European Nucleotide Archive (ENA) \cite{ENA2022} has a total of >2.7 billion assembled sequences as of 2022 \cite{ENAsite}. Often in medical applications and especially in bioinformatics, one needs to identify the species to which an observed DNA sequence belongs, which requires searching such genome archives. The sheer scale of these databases demands efficient sequence search algorithms. Bloom Filter(BF), a probabilistic data structure used for membership testing, \cite{BloomOriginalPaper}, and its variants \cite{bigSI,gupta2021fast, SSBT, Bingmann2019COBSAC, kmerBF}  are state-of-the-art data structures to efficiently search a given DNA sequence in petabytes of genomic data. Every DNA sequence in a genome is broken into $k$-length substrings, called k-mers, with a sliding window and then inserted into the bloom filter. The query is also divided into k-mers, and the membership of each k-mer is tested using BF. This is illustrated in figure \ref{fig:kmerBFInsert}.

% what RH lacks sequence search in BF.
RH functions are critical to the success of Bloom filters used in membership testing problems. Typical membership testing problems have queries of the form ``$q \in A?$" where set $A$ is fixed. BF uses a bit-array, each bit of which is set to 1 if some element of $A$ hashes to it using an RH function. This bit-array is a representation of the set $A$. To check if $q$ is present in $A$, we hash $q$ using the same RH function and check if the bit at this location is set. In gene sequence search, we have to perform a sequence of membership testing queries for each k-mer of the query DNA sequence. In this case, RH has some undesirable properties. RH, being agnostic to the sequence of queries, distributes them randomly, causing us to fetch different caches (alt. pages in case of numa / disk access) for each subsequent query. This is a highly inefficient usage of the cache line (alt. page), where only one bit is used. Ideally, we want to colocate the bits for subsequent queries to utilize the cache line (alt. page) effectively. While LSH seems to have the required property to colocate the subsequent query k-mers, LSH will cause them to collide and thus lose the identity of k-mers. This situation highlights the need for hash function families that cater to the spectrum between LSH and RH. This paper discusses such a family of functions, namely \name hash, which can colocate subsequent k-mers while maintaining their identity.


% Universal hash has been used extensively in a probabilistic data structure called Bloom filter. It is a space-efficient set membership testing utility with wide applications. 
% % in networking, distributed databases, and genomic search. 
% Specifically, Bloom filter-based indices have proven to be state of the art for gene string search\cite{bigSI} \cite{gupta2021fast} \cite{SSBT} \cite{Bingmann2019COBSAC}. 
% It encodes a big gene string ($\approx 100M$) \cite{gupta2021fast} with a kmer-based set representation. Like an n-gram token for a text, kmer is a $k$ length token generated using a sliding window of stride one on the gene (Figure \ref{kmerBFInsert} )\cite{kmerSelection}. A query gene as a sequence of kmers can be checked quickly for its presence by querying each kmers. The UH with Bloom filter has shown superior search and indexing of the genome sequences; however, the random bit accesses lead to many cache misses \ref{fig:ckbf}. This motivated a hash function that preserves identity like UH and keeps the similar kmers in gene sequence together (like LSH) to reduce the cache misses. 

% % It is a membership tester that provides quick search results in cheap memory\ref{fig:BFdataStr}. 
% \paragraph{Indexing Genomic data:}
% Genomic data is a set of specie specific files (represented as .fasta/.fastq), containing a lengthy sequence of basepairs- A, T, C, and G. The European Bioinformatics Institute (EBI) has reportedly stored around 160 Petabytes of raw DNA sequences as of 2018 \cite{EBI2019}. The European Nucleotide Archive (ENA) \cite{ENA2022} has a total of >2.7 billion assembled sequences as of 2022. This sheer scale demands efficient sequence databases and search algorithms. Any file-based inverted index is far from useful as a sample of 10000 files contains $2.2 \times 10^10$ distinct tokens (called kmers) \cite{Bingmann2019COBSAC}, making it impractical to store the dictionary. Even a minimal perfect hash needs prior distribution knowledge of kmers, and the index can very easily take more than $100 TB$ \ref{appendix} \gaurav{
% provide calculation in appendix:\\
% $\Gamma_{mph} \times (2.2 \times 10^10)\times PointerSize \\
% \times AvgNumFilesPerKmer \times FilePrecision \\
% = 2 \times (2.2 \times 10^10)\times 8 \times 100 \times 4 = 128TB$
% } of storage against $<150 GB$ for a simple Array of Bloom filter \cite{Bingmann2019COBSAC}. Having millions of species files against trillions of kmers, a Bloom filter encoding every file as a kmer-based representation is much more space-friendly, modular, and fast\cite{gupta2021fast}. 

\longname(\namens) family strikes a balance between RH and LSH families, and provides the best of both worlds. It colocates the values of similar input tokens but does not cause them to collide, thus preserving their identity. Additionally, it randomly distributes dissimilar tokens across the range. We give a general construction of \name functions using LSH and RH functions. We generalize the Bloom filter by replacing traditional RH functions with \name functions. The Bloom filter with \name hash function, called \name-BF, is suitable for efficient sequential querying operations. In the context of genomic search, we design a \name-BF which makes the subsequent k-mer in the DNA sequence colocate in a range without colliding. Thus, when a cache line  (alt. page) is fetched to access the bit of the current k-mer, with high probability, the same cache line  (alt. page) also contains the bit for subsequent k-mer. Thus, \name-BF reduces cache misses (alt. page-faults)  and improves the latency of indexing and querying DNA sequences. 

We describe the \longname(\namens) hash family and provide a general recipe to construct \name functions in section \ref{sec:family}. Design of \name function for gene search, and its efficient implementation is described in section \ref{sec:genesearch}. We analyse the false positive rate of \name-BF in section \ref{sec:analysis} and perform extensive evaluation in section \ref{sec:exp} Our experiments verify the effectiveness of \name-BF for gene search, and show that we slash our index and query times on RAM and query times on disk by over 30\% when compared to state-of-the-art BF while achieving the same false positive rates. 

%\apd{summarize todo after experiments section.}


% To summarize-

% \begin{itemize}
%     \item We provide a new class of hash function - \longname(\namens). It preserves locality among similar keys and the identity of each key.
%     \item We propose \name -Bloom Filter for gene sequence indexing and search. It improves the Insert and Query time by a factor of --- on RAM and --- on disk.
%     \item We provide a complete theoretical analysis of the false positive rate for \name -BF.
%     \item With \name -BF, we attain a Multiple Set Membership Testing query and insert improvements of ----.    
% \end{itemize}


% Bloom filter encodes a fastq file with a kmer-based gene representation. Like an n-gram token for a text, kmer is a $k$ length token generated using a sliding window of stride one on the gene \ref{fig-kmer} \cite{}. 
% With this, the gene sequence is encoded as a set in a Bloom Filter. A single gene sequence can be as large as X billion for -- and usually 50-200M in length in a single parasite and bacteria.









==> sections/introduction_2.tex <==
% RH and LSH are super useful.  

Retrieval and search systems in practice are often deployed to serve a batch of queries. This is specifically non-limiting when a single input from the user is translated into a group of small queries. It happens exactly in gene sequence search. The query gene (a string of DNA sequence, e.g., ATCGTCAACTGA..)is divided into a set of $k$ size tokens called kmers\cite{kmerSelection,bigSI}. For a typical query of size $100$ to $500$, the batch size is $101-k$ to $501-k$, attributed to the fact that the kmer are selected from a sliding window of stride 1. This is necessary for highly accurate genomic queries. The SOTA search engines \cite{SSBT,kmerBF} employ a Random hash (RH) based approach to query these kmers from a Bloom filter (BF). The randomness of the hash provides the best False positive rate guarantees on BF. However, this randomness leads to many cache misses (alt. page faults) in the process of addressing a batch of query kmers. The sliding window of stride 1 - based kmer selection provides a high intra-batch similarity in the query. This opens up a gateway to address the cache misses. The bioinformatics analysis is accuracy critical, and the identity of a kmer is highly significant. Among the stringent requirements of exactness, along with the blessing of intra-batch similarity, there is a possibility for a new hash function that can cater to genomic search with reduced cache misses, keeping very low error rates.  

Hash functions have been widely used in big data systems\cite{practicalML,b3}, network and security\cite{BFsurvey}, and AI\cite{MACH}. Specifically, Random hash (RH) and its proxies \cite{universalHashcarter1979, murmur, xxHash}, and Locality sensitive hash functions (LSH) \cite{IndykAndMotwani} has created a wave of improved probabilistic data structures which have provided exponential improvements in memory and speed with an insignificant cost of uncertainty\cite{NIPS2011_anshu}. Thus, it comes as no surprise that LSH and RH have helped to achieve performant algorithms in multiple domains, including but not limited to sampling \cite{ioffe2010improved}, retrieval \cite{IndykAndMotwani, wang2017flash, gupta2022bliss, baeza1999modern} and machine learning \cite{ryanDeepLeanring, chen2020slide}. The recent advancement in the genomic search \cite{elworth2020petabytes, bigSI} index, catering to hundreds of Terabytes of data \cite{gupta2021fast}, has been attributed to the RH and LSH functions. Especially RH functions, which are good at maintaining the identity of the input. 
If two input keys are distinct, with high probability, the RH function will map it to two separate keys. This is an obligation for gene sequence search as even a single base-pair change can lead to different biological behaviors \cite{lee2020unique}. RH maintains the input's identity; however, as it maps a key uniformly randomly and independently to an integer in $[m] ={0,1,2...m-1}$, the batch of keys will face high cache misses during a READ or WRITE on the memory.  

A locality-sensitive hash (LSH) function is used to collide similar inputs. The LSH gives the same value to similar keys with high probability and avoids assigning the same value for different keys. It has been proven very efficient for near neighbor search \cite{IndykAndMotwani} \cite{shrivastava2014asymmetric} and deep learning \cite{chen2020slide}. LSH provides locality!; hence it can be used for hash colocation in the cache. While it is an encouraging thought for genomic search, its strength is also a weakness here. As LSH will map similar kmers to a single value, it will not preserve the identity of these kmers. 

In some sense, RH and LSH lie at two ends of a spectrum. LSH combines similar elements, causes them to have identical values, and induces a lapse of identity; RH preserves identity but at the cost of being agnostic to any similarity. In this paper, we provide a new hash family \longname(\name hash) that offers a way to achieve the complete spectrum between LSH and RH. This way, we achieve gene identity with cache locality and show the improvement on  search in genomic data with our proposed \name hash function and \name- Bloom filter.

\paragraph{Gene Sequence search:} The genome of an organism is the complete set of DNA for that organism. The DNA sequence readers \cite{goodwin2016coming} aim to determine the nucleic acid sequence (A, C, T, and G) of a gene. The genome archives recording such sequences for multiple species are typically very large. For instance, the European Bioinformatics Institute (EBI) has reportedly stored around 160 Petabytes of raw DNA sequences as of 2018 \cite{EBI2019}. Additionally, the European Nucleotide Archive (ENA) \cite{ENA2022} has a total of >2.7 billion assembled sequences as of 2022 \cite{ENAsite}. Often in medical applications and especially in bioinformatics, one needs to identify the species to which an observed DNA sequence belongs, which requires searching such genome archives. The sheer scale of these databases demands efficient sequence search algorithms. Bloom Filter(BF), a probabilistic data structure used for membership testing, \cite{BloomOriginalPaper}, and its variants \cite{bigSI,gupta2021fast, SSBT, Bingmann2019COBSAC, kmerBF}  are state-of-the-art data structures to efficiently search a given DNA sequence in petabytes of genomic data. Every DNA sequence in a genome is broken into $k$-length substrings, called k-mers, with a sliding window and then inserted into the bloom filter. The query is also divided into k-mers, and the membership of each k-mer is tested using BF. This is illustrated in figure \ref{fig:kmerBFInsert}.

\input{figures/kmerinsert}

% what RH lacks sequence search in BF.
RH functions are critical to the success of Bloom filters used in membership testing problems. Typical membership testing problems have queries of the form ``$q \in A?$" where set $A$ is fixed. BF uses a bit-array, each bit of which is set to 1 if some element of $A$ hashes to it using an RH function (Section \ref{sec:background}). This bit-array is a representation of the set $A$. To check if $q$ is present in $A$, we hash $q$ using the same RH function and check if the bit at this location is set. In gene sequence search, we have to perform a sequence of membership testing queries for each k-mer of the query DNA sequence (Figure \ref{fig:kmerBFInsert}). In this case, RH is not fully justified. RH, being agnostic to the sequence of queries, distributes them randomly, causing us to fetch different caches (alt. pages in case of numa / disk access) for each subsequent kmer in the query. This is a highly inefficient usage of the cache line (alt. page), where only one bit is used. Ideally, we want to colocate the bits for subsequent queries to utilize the cache line (alt. page) effectively. While LSH seems to have the required property to colocate the subsequent query k-mers, LSH will cause them to collide and thus lose the identity of k-mers. This situation highlights the need for hash function families that cater to the spectrum between LSH and RH. In section \ref{sec:family}, we introduce such a family of functions, namely \name hash, which can colocate subsequent k-mers while maintaining their identity.

\longname(\namens) family strikes a balance between RH and LSH families, and provides the best of both worlds. It colocates the values of similar input tokens but does not cause them to collide, thus preserving their identity. Additionally, it randomly distributes dissimilar tokens across the range. We give a general construction of \name functions using LSH and RH functions. We generalize the Bloom filter by replacing traditional RH functions with \name functions. The Bloom filter with \name hash function, called \name-BF, is suitable for efficient sequential querying operations. We design a \name-BF for gene sequence search, which makes the subsequent k-mer in the DNA sequence colocate in a range without colliding. Thus, when a cache line  (alt. page) is fetched to access the bit of the current k-mer, with high probability, the same cache line  (alt. page) also contains the bit for subsequent k-mer. Thus, \name-BF reduces cache misses (alt. page-faults)  and improves the latency of indexing and querying  on DNA sequences. 

Section \ref{sec:family} describes the proposed \longname(\namens) hash family and provides a general recipe to construct \name functions. The design of \name function for gene search and its efficient implementation is described in section \ref{sec:genesearch}. We analyze the false positive rate of \name-BF in section \ref{sec:analysis} and perform the extensive experimental evaluation in section \ref{sec:exp}. Our experiments verify the effectiveness of \name-BF for gene search and show that we slash our index and query times on RAM (\gaurav{by 40\% and 30\% respectively} ) and query times on disk by over 30\% when compared to state-of-the-art BF while achieving the same false positive rates. 

%\apd{summarize todo after experiments section.}


% To summarize-

% \begin{itemize}
%     \item We provide a new class of hash function - \longname(\namens). It preserves locality among similar keys and the identity of each key.
%     \item We propose \name -Bloom Filter for gene sequence indexing and search. It improves the Insert and Query time by a factor of --- on RAM and --- on disk.
%     \item We provide a complete theoretical analysis of the false positive rate for \name -BF.
%     \item With \name -BF, we attain a Multiple Set Membership Testing query and insert improvements of ----.    
% \end{itemize}


% Bloom filter encodes a fastq file with a kmer-based gene representation. Like an n-gram token for a text, kmer is a $k$ length token generated using a sliding window of stride one on the gene \ref{fig-kmer} \cite{}. 
% With this, the gene sequence is encoded as a set in a Bloom Filter. A single gene sequence can be as large as X billion for -- and usually 50-200M in length in a single parasite and bacteria.









==> sections/introduction_3.tex <==
Data mining systems heavily rely on hash functions\cite{practicalML,b3}: functions that map arbitrary size values to a fixed range $[m]=\{0,..{m-1}$. For instance, some fundamental data structures used for search and estimation problems are a hash table, bloom filters\cite{bloom1970space}, count-sketches\cite{cormode2005improved}, etc., which use random hash(RH) functions and their variants\cite{universalHashcarter1979, murmur, xxHash}. While RH and other hash functions have revolutionized search systems\cite{ioffe2010improved,IndykAndMotwani, wang2017flash, gupta2022bliss, baeza1999modern, bigSI, elworth2020petabytes,practicalML, ryanDeepLeanring} by allowing us to build probabilistic data structures that exponentially improve memory and computational requirements, they are not conducive for system performance. Search systems often serve a batch of queries, and RH functions deployed in such systems map each query independently, and can lead to system inefficiencies such as high cache-miss rates and page faults. The general problem of processing a burst of queries with a random underlying pattern of memory access has received little attention. This paper considers a specific search system: gene sequence search, and highlights the issue associated with using the RH function from a system perspective. 

The problem of gene sequence search is identifying the species to which the given gene sequence belongs. Each specie is represented by its genome: the complete set of DNA sequences  (typically represented as a sequence of ``ACGT" characters)for that organism. The genome archives recording such sequences for multiple species are typically extensive. For instance, the European Bioinformatics Institute (EBI) has reportedly stored around 160 Petabytes of raw DNA sequences as of 2018 \cite{EBI2019}. Bloom Filter(BF), a probabilistic data structure used for membership testing, \cite{BloomOriginalPaper}, and its variants \cite{bigSI,gupta2021fast, SSBT, Bingmann2019COBSAC, kmerBF}  are state-of-the-art data structures to efficiently search a given DNA sequence in petabytes of genomic data. The search proceeds as follows. Each sequence of DNA is broken into k-mers using a sliding window of size $k$ and stride 1 (see figure \ref{fig:kmerBFInsert} for illustration), and each k-mer is sequentially queried for membership inside the bloom-filters built over the DNA database. Thus, each sequence search leads to a burst of queries to BF. RH functions, the primary reason for the success of BFs, being agnostic to the sequence of queries, distributes them randomly, causing us to fetch different caches/pages for each subsequent query. This is a highly inefficient usage of the cache /page, where only one bit is used from each fetch. Ideally, we want to colocate the bits for subsequent queries to utilize the cache and page mechanisms effectively. 
\input{figures/kmerinsert}

One alternative might be to consider locality-sensitive hash (LSH) functions\cite{IndykAndMotwani} 
that recognize the similarity between subsequent queries. However, the biggest strength of LSH in mapping similar tokens to the same value is a weakness in this scenario. As LSH maps similar keys to a single value, it does not preserve the identity of these keys. RH and LSH lie at two ends of a spectrum. LSH combines similar elements, causes them to have identical values, and induces a lapse of identity; RH, on the other hand, preserves identity but at the cost of being agnostic to any similarity. However, to improve gene-search system performance, we need a hash function that draws properties from both RH and LSH. In this paper, we provide a new hash family \longname(\name) that offers a way to achieve the complete spectrum between RH and LSH. 

\longname(\namens) family strikes a balance between RH and LSH families and provides the best of both worlds. It colocates the values of similar input tokens but does not cause them to collide, thus preserving their identity. Additionally, it randomly distributes dissimilar tokens across the range.(see figure \ref{fig:lphcollision}) We give a general construction of \name functions using LSH and RH functions. We generalize the Bloom filter by replacing traditional RH functions with \name functions. The Bloom filter with \name hash function, called \name-BF, is suitable for efficient sequential querying operations. In the context of genomic search, we design a \name-BF which makes the subsequent k-mer in the DNA sequence colocate in a range without colliding. Thus, when a cache line  (alt. page is accessed) is fetched to access the bit of the current k-mer, with high probability, the same cache line/page also contains the bit for subsequent k-mer. Thus, \name-BF reduces cache misses/page faults and improves the latency of indexing and querying DNA sequences. 

We describe the \longname(\namens) hash family and provide a general recipe to construct \name functions in section \ref{sec:family}. The design of \name function for gene search and its efficient implementation is described in section \ref{sec:genesearch}. We analyze the false positive rate of \name-BF in section \ref{sec:analysis}. This analysis can be of independent theoretical interest. Also, we perform an extensive evaluation in section \ref{sec:exp}. Our experiments verify the effectiveness of \name-BF for gene search. We see about $2 \times$ speedup in indexing and query times with \name hashing while maintaining the same false positive rates for BF. With an Array of BF, we get about $1.5\times$ indexing and query speed up for the same.


==> sections/method.tex <==
\section{Fuzzy Locality Sensitive hash}
% The Locality sensitive hash ensures a high probability of collision of similar key.
The Fuzzy LSH ensures the adjacency of similar keys with a high probability (Figure \ref{fuzzyHashGeneric}). Formally the fuzzy-LSH provides the following hash property-
\begin{theorem}
        A family  $\mathcal{F}$ is called
                $(r,cr,p_1,p_2,L)$ fuzzy sensitive if for any two points $x,y \in \mathcal{U}$ and $h$ chosen uniformly from $\mathcal{H}$ satisfies the following:\\
            if $Dist(x,y)\le r$ then 
                 \begin{itemize}
                    \item  ${Pr}(\Delta_1\leq|h(x)- h(y)|\leq \Delta_2) \ge p_1\frac{(2\Delta_2 -2\Delta_1 +1)}{L}$
                    \item ${Pr}(h(x)= h(y)) \le \frac{1}{L}$
                \end{itemize} 
                \\
            if $ Dist(x,y)\ge cr$ then 
             \begin{itemize}
                    \item  ${Pr}(\Delta_1\leq|h(x)- h(y)|\leq \Delta_2) \le p_2\frac{(2\Delta_2 -2\Delta_1 +1)}{L}$
                     \item ${Pr}(h(x)= h(y)) \le p_2\frac{1}{L}$
                \end{itemize}
                \label{def:fuzzylsh}
\end{theorem}

Where $h(.) \in [1,m]$.  $\Delta_1, \Delta_2 \in [0,L/2 -1]$, is the hash location gap in the neighborhood of $L$ and $L< m$.
Here, the similar keys fall within a small distance $\Delta = \Delta_2 -\Delta_1$ from each other, keeping a low probability of colliding in the same place.

\todo{review above. The upper bound ${Pr}(h(x)= h(y)) \le \frac{1}{L}$ is loose. }

\section{Cache Efficient Kmer Bloom Filter - CKBF}
\subsection{Intuition}
The universal hash function provides independent and uniform collision probability for every key. With this, any two distinct kmers in the gene sequence will get hash values independent of each other. A Write or Read on these memory locations is done by loading the entire cache line into the CPU cache. Usually, this benefits when the cached data is used entirely for the computation. However, the Bloom filter only needs the corresponding bit access, wasting the rest of the cache most of the time. 

The Fuzzy Locality Sensitive hash provides nearby hash locations for similar kmers (Figure \ref{cacheMotivation}). A significant overlap between any two kmers is more likely to be neighbors in the gene sequence. For example, 
adjacent kmers differ by two base pairs and hence have high similarity. Fuzzy hash exploits this in favor of query time by combining a locality-sensitive hash and a universal hash. The locality-sensitive hash value provides the address in the units of cache line size and the universal hash provides an independent hash location with a maximum range of cache line size. \todo{can replace cache-line with block}. 

\subsection{Fuzzy Locality Sensitive hash for sequence}
The Fuzzy Locality Sensitive hash for sequence is formally defined as-

We use minhash \cite{} function to get the locality-sensitive hash representing a gene text string 
\begin{definition}
For a given kmer $x$ of length $k$, the fuzzy LSH is given by
$$h_f(x) = L*h_m(x)mod  \left \lceil{\frac{m}{L}}\right \rceil + h_u(x)mod L$$
\end{definition}
Where $ h_m(x)$ is the minhash \cite{} of the kmer string defined as-
$$ h_m(x) = min \left(h_u(x_1),h_u(x_2), ...h_u(x_{k-d+1})\right) $$
The $x_1..x_{K-d+1}$ are the minhash tokens of $x$, $h_u(.)$ is the universal hash, $L$ is the cache-line size and $m$ is the total range.

\begin{algorithm}
% \setstretch{1.14}
\begin{algorithmic}
% \SetAlgoLined
\STATE {\bf Input:} Set of kmers $x_1...x_n$ from a gene sequence $S$, 
\STATE  \ \ \     $h_u(.)$ universal hash
\STATE {\bf Result:} $h_f(x)$
\FOR{term $i \in $ $1..n$}
    \STATE $ h_m(x) = \min_{j} \left(h_u(x_{i,j})\right) , j \in \{1..k-d+1\} $
    \STATE $h_m(x) = L*h_m(x)mod  \left \lceil{\frac{m}{L}}\right \rceil$
\ENDFOR  
\STATE $ h_f(x) = h_m(x) +  h_u(x) mod L$
    
 \end{algorithmic}
  \caption{Fuzzy LSH Algorithm}
  \label{alg:fuzzyLSH}
\end{algorithm}

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{imgs/rollingminhash.png}
  \caption{Rolling Minhash}
  \label{rollingminhash}
\end{figure}l

\subsubsection{Theory}
\begin{theorem}
Fuzzy LSH $h(x)$ collision probability: For all $x\neq y \in U$, 
% and the set size $\mathcal{S}(x)$ and $\mathcal{S}(y)$ atleast $c\log \frac{1}{\epsilon}$ 

$$\Pr _{h_f\in {\mathcal {H}_f}}[ h_f(x)= h_f(y)]= \frac{1}{L}\left(\frac{1}{\left \lceil{m/L}\right \rceil} + \left(1- \frac{1}{\left \lceil{m/L}\right \rceil} \right){\frac {|\mathcal{S}(x)\cap \mathcal{S}(y)|}{|\mathcal{S}(x)\cup \mathcal{S}(y)|}}\right)$$

Where $m$ is the range of fuzzy LSH, $L$ is the parameter defining the cache line size, and $\mathcal{S}(x)$ represents the minhash token set of $x$.

\end{theorem}

\begin{lemma}
For kmer strings $x_i$ and $y_i$ of length $k$ each, such that $x_i$ and $y_i$ differs by at-least 1 base-pair, the Jaccard similarity $J(.)$ of the corresponding token sets $\mathcal{S}(x_i)$ and $\mathcal{S}(y_i)$ is bounded by 
$$ \Pr _{h_m\in {\mathcal {H}_m}}[ J(x_i)= J(y_i)] \in \left(0, \frac{k-d}{k+2-d}\right)$$, 
Where $d$ is the token size.
\end{lemma}


\todo{If we assume circular subkmer token generation the upper bound reduces, I would suggest to use this bound
$$ \Pr _{h_m\in {\mathcal {H}_m}}[ h_m(x)= h_m(y)] \in \left(0,\frac{k+1-2d}{k+1}\right)$$}
% with exact 1 basepair difference it is
% $$ \Pr _{h_m\in {\mathcal {H}_m}}[ h_m(x)= h_m(y)] \in \left(\frac{k+1-2d}{k+1}, \frac{k-d}{k+2-d}\right)$$, 

The highest fuzzy LSH collision probability if kmers $x_i\neq y_i$ is
$$\Pr _{h_f\in {\mathcal {H}_f}}[ h_f(x)= h_f(y)]= \frac{1}{L}\left(\frac{1}{\left \lceil{m/L}\right \rceil} + \left(1- \frac{1}{\left \lceil{m/L}\right \rceil} \right){\frac{k+1-2d}{k+1}}\right)$$


\subsection{Insert and query}
The Cache efficient Kmer Bloom filter uses the Fuzzy LSH for sequence insertion and query. For a given gene sequence, a single-stride sliding window generates the kmers to represent the entire sequence as a set.

\begin{algorithm}
% \setstretch{1.14}
\begin{algorithmic}
% \SetAlgoLined
\STATE {\bf Input:} Gene sequence $S$, $h_f(.)$ fuzzy hash function
\STATE {\bf Result:} CKBF (size: $m$ )
\FOR{kmer $x \in $ $\mathcal{S}$}
        \STATE $CKBF[h_f(x)]=1$
\ENDFOR
% \WHILE{Input $S_i$}
%     \FOR{term $x \in $ $S_i$}
%         \FOR{$d = 1, ... R$}
%             \STATE Insert($x$, CKBF[$ \phi_d(x),d$])
%         \ENDFOR
%     \ENDFOR 
% \ENDWHILE
 \end{algorithmic}
  \caption{CKBF Sequence Insert and Query. \todo{To finish}}
  \label{alg:ckbf}
\end{algorithm}


% \begin{algorithm}
% % \setstretch{1.14}
% \begin{algorithmic}
% % \SetAlgoLined
% \STATE {\bf Input:} Set $\mathcal{S}$ of $K$ sets 
% \STATE {\bf Result:} RAMBO (size: $B \times R$ )
% \STATE Generate $R$ partition hash functions $\phi_1(\cdot), ... \phi_R(\cdot)$
% \STATE RAMBO $\leftarrow B\times R$ array of Bloom Filters
% \WHILE{Input $S_i$}
%     \FOR{term $x \in $ $S_i$}
%         \FOR{$d = 1, ... R$}
%             \STATE Insert($x$, RAMBO[$ \phi_d(x),d$])
%         \ENDFOR
%     \ENDFOR 
% \ENDWHILE
%  \end{algorithmic}
%   \caption{CKBF Sequence Insert and Query}
%   \label{alg:ckbf}
% \end{algorithm}

\subsubsection{Theory}
\gaurav{Needs brainstorming}

\subsubsection{Query time}
hash time :
$$ \eta n(2t_u + \log (k-d+1))$$
$t_u$ is the universal hash calculation time, $\eta $ is number of hash functions, $k$ is the kmer length and $d$ is the token size.
check time :
$$O(\eta n/(Lp_L))$$
\gaurav{todo: find $Lp_L$: expected share of consecutive keys in width $L$ }


==> sections/problemdefinition.tex <==
The Membership testing and Multiple set membership testing of a gene sequence query $q$ is defined as-
\paragraph{Membership testing}
A gene sequence query $Q$ is present in a given larger gene sequence $S$ if the set of kmers $\mathcal{Q}$ from $Q$ is a subset of the set of kmers $ \mathcal{S}$ from $S$, i.e. $\mathcal{Q} \in \mathcal{S}$. For a given Bloom filter $\mathbb{B}$ constructed on $\mathcal{S}$, the membership $M(Q)$ is given by
$$ M(Q) = \mathbb{B}(h(q_1)) \land \mathbb{B}(h(q_2)) \land ...\mathbb{B}(h(q_k))   $$

\paragraph{Multiple set membership testing}
\todo{to change this}
We have given a set of query kmers $\mathcal{Q}$ tokenized from a gene sequence query and a set of $N$ membership testers, each representing the set of kmers $S_n \in \mathcal{S}$. 

The Multiple set membership testing (MSMT) aims to query all membership testers to identify the sets $A_q \subseteq \mathcal{S}$ containing the given query kmers$Q$.


==> sections/thm1proof_new.tex <==


\section{Proof of Theorem 1}
\begin{theorem} (general \name construction)
Let $\phi$ be drawn from a $(r_1, r_2, p_1, p_2)$ sensitive LSH family say $\mathcal{L}$ and $\rho_1, \rho_2$ be drawn from a random hash family, say $\mathcal{R}_1 : V \rightarrow [m], \mathcal{R}_2: U \rightarrow [L]$ respectively. Then the family of hash functions defined by 
\begin{equation}
    \mathcal{I} : \{\psi(x) = \rho_1(\phi(x)) + \rho_2(x)) \}
\end{equation}
is a $(r_1, r_2, \frac{L-1}{L}p_1, \frac{L}{m}+ p_2)$ sensitive and $L$ preserving {\longname } (\name) family.
\end{theorem}
If $d_U(x,y) \leq r_1$, then
\begin{proof}

\begin{align*}
    & \mathbf{Pr}(\mathbf{1}(\psi(x) \neq \psi(y)) \wedge d_V(x, y) < L ) \\
    & = \mathbf{Pr}(\phi(x) = \phi(y))\frac{L-1}{L} + \mathbf{Pr}(\phi(x) \neq \phi(y) \wedge (\textrm{satisfies the conditions}))\\
    & \geq \mathbf{Pr}(\phi(x) = \phi(y))\frac{L-1}{L} \\
    & = p_1 \frac{L-1}{L} 
\end{align*}

If $d_U(x,y) > r_2$, then,
\begin{align*}
    & \mathbf{Pr}( d_V(x, y) < L ) \\
    & = \mathbf{Pr}(\phi(x) = \phi(y)) + \mathbf{Pr}(\phi(x) \neq \phi(y) \wedge (\mathbf{Pr}(|\rho_1(x) - \rho_1(y)| < L) \wedge (\textrm{satisfies the condition}))\\
    & \leq p_2 + \mathbf{Pr}(\phi(x) \neq \phi(y) \wedge (\mathbf{Pr}(|\rho_1(x) - \rho_1(y)| < L)\\
    & \leq p_2 + (\mathbf{Pr}(|\rho_1(x) - \rho_1(y)| < L)\\
    & = p_2 + \frac{L}{m}\\
\end{align*}
\end{proof}






==> tables/hashes.tex <==
\begin{table}[]
\centering
\caption{The number of hash computations per k-mer for BF and \name-BF. With one-permutation hashing, rolling-min-hash computation and performing random hash function based MinHash, we only need to perform $\eta+1$ hash computations per k-mer for \name for all k-mers except first k-mer in the sequence. For the first k-mer we need to compute $\eta + (k-t+1)$ where $k$ is the k-mer length and $t$ is the sub-k-mer length.}
\label{tab:hashes}
\begin{tabular}{|c|c|}
\hline
                                      & \#hash comptuations per k-mer \\ \hline
BF($m, \eta$)                         & $\eta$                        \\ \hline
\name-BF($m, \eta, L$) & $\eta + 1$                    \\ \hline
\end{tabular}
\end{table}

==> trash/theory1.tex <==

Let us analyse the false positive rate for our Identity preserving distance sensitive Bloom Filter.

Let us consider a partitioned bloom filter of range $m$ and number of hash functions $k$, let $m' = m / k$. Consider the set of tokens $n = |S|$ which are inserted into the bloom filter. We will be using a generalized notion of distance-sensitive hash families, where given two tokens x, y, the probability of collision of these two tokens is bounded
\begin{equation}
    p_L(\zeta(x,y) \leq \mathbf{Pr}(h(x) = h(y)) \leq p_H(\zeta(x,y))
\end{equation}
The false positive rate for a token $u \notin S$ is
\begin{align*}
    \mathbf{Pr}(\textrm{all locations of }h_i(u) 
    \textrm{ are set})
\end{align*}

\begin{align*}
    \mathbf{Pr}(\textrm{ith of }h_i(u) 
    \textrm{ is  set})^k
\end{align*}
Let this probability be $p_u$
\begin{align*}
    p_u^k
\end{align*}
We need to find an upper bound on $p_u$. 
\begin{align*}
    p_u = \mathbf{Pr}( \mathbf{1}(h(u) == h(s_1)) \vee \mathbf{1}(h(u) == h(s_2)) \vee ... \vee \mathbf{1}(h(u) == h(s_n)))
\end{align*}
\textbf{Simplest analysis:} By union bound,
\begin{align*}
    p_u \leq \sum_i \left(p_H(\zeta(u, s_i)) \frac{1}{L} + \frac{1}{m'}\right)
\end{align*}

\begin{align*}
    p_u \leq \left( \frac{1}{L} \sum_i p_H(\zeta(u, s_i)) \right)  +  \frac{nk}{m}
\end{align*}

\begin{align*}
    p^k_u \leq \left(\left( \frac{1}{L} \sum_i p_H(\zeta(u, s_i)) \right)  +  \frac{nk}{m} \right)^k
\end{align*}

Note that for a arbitrary sequence of tokens $S$, this is a tight analysis as union bound is tight in case the events are disjoint.

We make the following observation from the above equation
\begin{itemize}
    \item In case of using jaccard similarity , if the average similarity is $s$, then 
    
    \begin{align*}
    p^k_u \leq \left(\left( \frac{ns}{L} \right)  +  \frac{nk}{m} \right)^k
    \end{align*}
    Thus, we need to choose $L$ that is greater than $ns$ to get something reasonable. The choice of $L$ depends on the relation of $u$ to the elements in the set $S$
    \item It should be noted that direct comparison of the above equation with standard bloom filter analysis will lead to pessimistic estimates of $m$ for a given k. This would come from the fact that standard bloom filters assume perfect random hash function. and in some sense this analysis is 1st order approximation of that analysis. So we would end up with exponentially more estimates of $m$ for FuzzyBF to get comparative FPR.
\end{itemize}

\paragraph{Realistic scenario}
\begin{itemize}
    \item Let us look at the moving window in sequence tokenization which is relevant to our case. Let the total length be $n$, let the window be $w$.
    \item If two tokens are from different parts and have no overlap, then the similarity between them is 0. And hence the probability of collision (before random hash to range) is 0.
\end{itemize}

\begin{align*}
    p_u = \mathbf{Pr}( \mathbf{1}(h(u) = h(s_1)) \vee \mathbf{1}(h(u) = h(s_2)) \vee ... \vee \mathbf{1}(h(u) = h(s_n)))
\end{align*}
Let the set $S_{a:b}$ denote the subset of elements $\{s_a,s_{a+1}, ... s_{b-1}\}$. Also, the even that $u$ collides with $S_{a:b}$ be $\mathbf{1}(h(u) \in h(S_{a:b})$
Then we can write this as, 
\begin{align*}
    p_u = \mathbf{Pr}( \mathbf{1}(h(u) \in h(S_{0:w}) \vee \mathbf{1}(h(u) \in h(S_{w:2w}) \vee .. \vee \mathbf{1}(h(u) \in h(S_{n-w:n}) )
\end{align*}
Applying union bound on the alternating sets,
\begin{align*}
    p_u \leq \mathbf{Pr}( \mathbf{1}(h(u) \in h(S_{0:w}) \vee \mathbf{1}(h(u) \in h(S_{2w:4w}) \vee ..) + \mathbf{Pr}( \mathbf{1}(h(u) \in h(S_{w:2w}) \vee \mathbf{1}(h(u) \in h(S_{3w:5w}) \vee ..)
\end{align*}

\begin{align*}
    p_u \leq \left(1 -  \Big( \mathbf{Pr} \left( \mathbf{1}(h(u) \notin h(S_{0:w}))\right)  
    \mathbf{Pr} \left( \mathbf{1}(h(u) \notin h(S_{2w:4w}))\right) ...
    \Big) \right)
     \\ 
    + \left(1 -  \Big( \mathbf{Pr} \left( \mathbf{1}(h(u) \notin h(S_{w:2w}))\right)  
    \mathbf{Pr} \left( \mathbf{1}(h(u) \notin h(S_{3w:5w}))\right) ...
    \Big) \right)
\end{align*}

\begin{align*}
    p_u \leq \left(1 -  \left( \prod_k \Big( \mathbf{Pr} \left( \mathbf{1}(h(u) \notin h(S_{2kw:2(k+1)w}))\right) \Big) \right) \right)
     \\ 
    + \left(1 -  \left( \prod_k \Big( \mathbf{Pr} \left( \mathbf{1}(h(u) \notin h(S_{(2k+1)w:(2k+3)w}))\right) \Big) \right) \right)
\end{align*}

\begin{align*}
    p_u \leq \left(1 -  \left( \prod_k \Big( 1 -  \mathbf{Pr} \left( \mathbf{1}(h(u) \in h(S_{2kw:2(k+1)w}))\right) \Big) \right) \right)
     \\ 
    + \left(1 -  \left( \prod_k \Big( 1 - \mathbf{Pr} \left( \mathbf{1}(h(u) \in h(S_{(2k+1)w:(2k+3)w}))\right) \Big) \right) \right)
\end{align*}

Approximating using union bound,

\begin{equation}
    \mathbf{Pr} ( (h(u) \in h(S_{a:b})) \leq \sum_{a:b} \mathbf{Pr}(h(u) = h(s_i)) \leq \sum_i \left( \frac{p_H(\zeta(u,s_i)}{L} ) + \frac{1}{m'}\right)
\end{equation}


\begin{align*}
    p_u \leq \left(1 -  \left( \prod_k \Big( 1 - \frac{w}{m'} - \sum_{i \in 2kw:2(k+1)w} \frac{p_H(\zeta(u, s_i))}{L}\Big) \right) \right)
     \\ 
    + \left(1 -  \left( \prod_k \Big( 1 - \frac{w}{m'} - \sum_{i \in (2k+1)w:(2k+3)w} \frac{p_H(\zeta(u, s_i))}{L}\Big) \right) \right)
     \\ 
\end{align*}

\textbf{Pessimistic view 1:} If we bound the max (over subsets) "average (over the particular subset)" similarity of the query to the subset be $\rho$. In the following $k$ is again number of hash functions

\begin{align*}
    p_u \leq 2 \left(1 -  \left( \prod_k \Big( 1 - \frac{wk}{m} - \frac{w\rho}{L} \Big) \right) \right)
     \\ 
\end{align*}


\begin{align*}
    p_u \leq 2 \left(1 - \Big( 1 - \frac{wk}{m} - \frac{w\rho}{L} \Big)^{\frac{n}{2w}} \right)
     \\ 
\end{align*}

\begin{align*}
    p_u \leq 2 \left(1 - \Big( 1 - \frac{wk}{m} - \frac{w\rho}{L} \Big)^{\frac{n}{2w}} \right)
     \\ 
\end{align*}

Thus the final false positive rate is ,

\begin{align*}
    p_u^k \leq 2 \left(1 - \Big( 1 - \frac{wk}{m} - \frac{w\rho}{L} \Big)^{\frac{n}{2w}} \right)^{k}
     \\ 
\end{align*}

\textbf{Under the assumption that smaller tokens should be present in order for there to be similarity and that there is not similarity across subsets defined above} There is only one set where the similarity exists and let $\rho$ be the max similarity.

\begin{align*}
    p_u^k \leq 2 \left(1 - \Big( 1 - \frac{wk}{m} - \frac{w\rho}{L} \Big) \Big( 1 - \frac{wk}{m} \Big)^{ \left( \frac{n}{2w} -1 \right) } \right)^{k}
     \\ 
\end{align*}

